Personal Data Protection in Smart Home Activity Monitoring for Digital Health: A Case Study

Researchers in pervasive computing have worked for decades on sensor-based human activity recognition (HAR). Among the digital health applications, the recognition of activities of daily living (ADL) in smart home environments enables the identification of behavioral changes that clinicians consider as a digital bio-marker of early stages of cognitive decline. The real deployment of sensor-based HAR systems in the homes of elderly subjects poses several challenges, with privacy and ethical concerns being major ones. This paper reports our experience applying privacy by design principles to develop and deploy one of these systems.

==> Old/solutionV1.tex <==
\subsection{IRB approval and informed consent}
The project pilot has been approved by the reference IRB (ethical committee) for the hospital recruiting the subjects. The approval was based on a detailed description of the data being acquired, the data analysis being performed, the use of the data, and the forms for informed consent that the participating subjects have to sign. The details of the technical solutions for data protection were postponed to a future analysis which is the subject of the current document.

\subsection{ Data protection techniques}
The main privacy-preserving technique adopted in this pilot is pseudonymization and its effectiveness strongly depends on the proper identification of identifiers and quasi-identifiers as presented above. A second principle that we follow is the Separation of Duties: we assign different tasks to different entities, each one with a partial visibility of the data. In order to enforce this principle an authorization system based on access control must be implemented. This also enables a strict control of the data flow between the different data processors.
\subsubsection{Pseudonymization}: Pseudonymization refers to the process
of transforming and replacing identifying data with a string or number that cannot be linked to the original data without access to a specific secret. Various pseudonymization techniques can be employed based on system requirements, such as counters, random number generation (RNG), cryptographic
hash functions, message authentication codes (MAC), symmetric encryption, etc. Recent international guidelines on data pseudonymization as provided for example in [1] and [2].

\subsubsection{Authorization, access control, and Logging}: The system defines distinct roles (HOS, UniMi, IIT, IMT, TelMed, and external processors) and assigns specific permissions to each, granting access to only the necessary data for each role. Access is based on the tasks each role performs and the responsibilities they hold. By implementing this Role-Based Access Control (RBAC) system, data is securely managed. Each entity is restricted to accessing only the information required for its specific function, reducing the risk of unauthorized access or data breaches. Any access to the mapping between PIDs and subject identifiers as well as the download of sensitive data must be authorised based on an authentication system that should guarantee that the entity making the access has the right for the requested operation. The access needs to be logged with timestamp, type of access, and identifier of the entity that made the access.

\subsection{Dataflow architecture and protocols}

A backend system installed on a trusted infrastructure (e.g., an approved telemedicine platform) is orchestrating the workflow providing some Web apps for authentication and front-end interaction. HOS, upon authentication, can see a list of currently enrolled patients, and for each patient, it can access personal details and access a dashboard with data analysis visualization. HOS can also insert data from a newly  recruited patient. In this case, the backend software generates a corresponding pseudonym (PID) and an installation number (I#). Any data in output from the home gateway (Home GW) and directed to Unimi for data analysis does not contain either explicit identifiers or quasi-identifiers, but only the PID. The installation number will be used for requests for interventions on the home sensing infrastructure without referring either to patient identification data or to the PID. Figure 1 shows how different kinds of data are transferred between entities. This drawing ignores the role of the TelMed entity that, for the time being, can be considered a module of HOS.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{img/dataflow-Page-3.drawio.pdf}
    \caption{The dataflow architecture}
    \label{fig:dataflow}
\end{figure}


\textbf{Initialization protocol:}

\begin{enumerate}
    \item Whenever HOS has a new participating subject with personal data D0, it authenticates itself to the system, generates a PID for that patient, and securely stores the association of PID and D0. An “installation request”  ticket is opened for the IIT with D0 and I\#.
    \item The IIT, when authenticated, will see the ticket and will schedule a first appointment with the subject to visit the apartment and plan the installation. As a result, the IIT will insert some information in the system including the apartment map with the number, type, and planned position of sensors. It will ack the completion through the installation ticket.
    \item The IMT, when authenticated will see the newly enrolled patient with a PID and an installation ticket opened for the corresponding I\#, but it will not have access to any identifying data.  The IMT will prepare the infrastructure equipment, including the HomeGW configured with the subject’s  PID, and, when ready, it will notify the IIT through the ticket.  
    \item The IIT, based on the open ticket, will get the infrastructure devices, schedule an appointment with the subject, and proceed with the installation. When the installation is done, IIT notifies IMT
    \item The  IMT will verify that the whole data acquisition system works as planned and will close the ticket.
    
\end{enumerate}


Intervention protocol: IMT securely stores I# with PID. Whenever IMT observes that some data is not being acquired as expected, the connection is interrupted or any other infrastructure is malfunctioning, it sends an intervention request with I\# to IIT that will send back a notification (with I\#) whenever the problem is solved. Tickets are always closed by the IMT after checking that the issue is solved. Pseudonymized DB: All sensitive data acquired by the Home GW is stored in a database associated with the subject’s PID. The local database is periodically transferred to a central DBMS on the backend in pseudonymized form and the results of data analysis are only associated with the PID. Pseudonymized data re-association: The mapping between the PID and the data that HOS uses to identify the subject is stored in a secure storage protected by cryptography (on a DBMS supporting Data Transparent Encryption), and will be used by HOS to visualize the data analysis results on a dashboard for the specific subject possibly joined with the subject’s medical records.

\subsection{ Retention policies}
The retention of sensitive data at the Home GW should be limited not only for storage limitation but more importantly for privacy reasons since it is possibly exposed to IMT. (The current retention is 1 month). The central DBMS will keep the data for the whole duration of the study. After the study, the data will be anonymized by deleting the association between PID and subject and by performing a further analysis about the risk of re-associating the data with a subject. The anonymized data will be available for further research studies

==> Old/solutionsV2.tex <==
\begin{comment}
Suggested structure for the section
Title "PRIVACY-PRESERVING SOLUTION AND ASSESSMENT"

1- Solutions
    1-1: Solution RB approval and informed consent
    1-2: Adopted techniques for adversary D0- D1- D2- D3
        1-2-1: Interial adversory
            Pseudonymization
            Authorization, access control, and logging
        1-2-2: External adversory
            Transparent Data Encryption
            HTTPS
    1-3: Privacy Preserving Analysis of Location and Trajectory data
    1-4: Data flow

2- Assessment ******* Ignored ********
3- Compliance with data protection regulations
4- Compliance with AI Act ***** Ignored ******
\end{comment}






\subsection{Data protection techniques}
The implemented techniques for protecting from tables D0, D1, D2, and D3 are presented in this subsection. The adopted technique for protecting D4 is presented in the next subsection.
\subsubsection{Internal Adversaries}
The main privacy preserving technique adopted in this pilot is pseudonymization and its effectiveness strongly depends on the proper identification of identifiers and quasi-identifiers as presented above. A second principle that we follow is the separation of Duties. We assign different tasks to different entities, each one with a partial visibility of the data. In order to enforce this principle an authorization system based on access control must be implemented. This also enables a strict control of the data flow between the different data processors. 


\begin{itemize}
    \item Pseudonymization:
    It transforms and replace identifying data with a combination of letters and numbers that cannot be linked to the original data without access to the key. The implemented system use from AES-256 as a symmetric encryption to implement pseudonymization~\cite{doi/10.2824/860099} and~\cite{UKICO2022}. The implemented encryption method get the identifier data and a nance as input and generate a corresponding pseudonym (PID) for each subject.
    \item Authorization: It is implemented in the system to verifies the users and their permissions~\cite{barkadehi2018authentication}. For this purpose, the system use from Keycloak as an open source authentication solution~\cite{thorgersen2021keycloak}.
    \item Access control: The system defines distinct roles (HOS, UniMi, IIT, IMT, TelMed, and external processors) and assigns specific permissions to access to only the necessary data~\cite{sandhu1998role}. Access is based on the tasks each role performs and the responsibilities they hold.
    \item Logging: all accesses to the system are logged with timestamp, type of access, and identifier of the entity that made the access. The system uses from PostgreSQL and Keycloak to provide a detailed logging mechanism.
    %Various pseudonymization techniques can be employed based on system requirements, such as counters, random number generation (RNG), cryptographic hash functions, message authentication codes (MAC), symmetric encryption, etc. Recent international guidelines on data pseudonymization as provided for example in~\cite{doi/10.2824/860099} and~\cite{UKICO2022}.
    % Any access to the mapping is authorised based on an authentication system.
\end{itemize}

\subsubsection{External Adversaries}
To provide privacy preserving of data against external adveraries, attempts are made to protect data during transmission and in data at rest steps.
\begin{itemize}
    \item Transparent Data Encryption (TDE): it provides a layer of security by automatically encrypting and decrypting data stored in the database for ensuring that sensitive data remains confidential even if unauthorized access to the database files occurs~\cite{sidorov2015transparent}. For this purpose, system use from Percona Transparent Data Encryption extension of PostgreSQL.
    \item Secure web: the system implement HTTPS to ensure encrypted communication between services and users.
    
\end{itemize}

\subsection{Privacy Preserving Analysis of D4}
\subsubsection{The Process of Collecting D4} 
The D4 (location and trajectory data) is collected through the subject’s Android or iOS phone and recorded by Google’s location service~\cite{zheng2015trajectory}. For this purpose, the subject’s phone, with location-enabled services, continuously tracks their location and records location coordinates, timestamps, and activity types (e.g., walking, driving). Then, Google periodically compiles this data into time series objects, which include places visited (specific locations the subject stayed for a while) and activity segments (movements between visiting locations). At the end of each month, these time series objects convert to a JSON and automatically uploaded to the trusted server (e.g., OneDrive).

\subsubsection{Objectives of the outdoor mobility analysis}

The primary goal that clinicians expect by monitoring activities outside the home is to identify deviations from normal habits. In this project, clinicians are interested in the following: 
\begin{itemize}
    \item Repeated deviations from the usual time spent outside the home: Unusually long or short periods spent away from home. We are interested in duration-per-day and event counting per day
    %\item Changes in the time-of-the-day or day-of-the-week in which the subject is out
    \item Changes in the places the subject frequently visits (e.g., the subject stops going to the usual grocery store and starts going to a closer one).
    %\item Changes in the transportation used by the subject to reach a frequently visited place (e.g., taking public transportation or car instead of walking). 
    \item Changes in the route taken to reach or come back from a frequently visited place (e.g., unusual longer route). 
    \item Identifying repeated "wandering" behavior: apparently irrational trajectories that suggest the subject may be lost or experiencing difficulty in navigating. 
    %\item The above changes of habit should be analysed considering the season and some weather conditions.
\end{itemize}

\subsubsection{D4 Data Protecting}
Since D4 can act as a pseudo-identifier, it need distinct attention~\cite{jin2022survey}. For this reason, the collected JSON file securely stored in the TDE-enabled table within the database. In the next step, a data analysis algorithms are designed to automatically analyze and return the answers to the questions of clinicians. The answers are very unlikely to reveal the subject’s identity. 

\color{black}


\subsection{Dataflow architecture and protocols}
A backend system installed on a trusted infrastructure (e.g., an approved telemedicine platform) is orchestrating the workflow providing some web apps for authentication and front-end interaction.
HOS, upon authentication, can see a list of currently enrolled patients, and for each patient, it can access personal details and access a dashboard with data analysis visualization. HOS can also insert data from a newly recruited patient. In this case, the backend software generates PID and an installation number (I\#). Any data in output from the home gateway (Home GW) and directed to Unimi for data analysis does not contain either explicit identifiers or quasi-identifiers, but only the PID. The installation number will be used for requests for interventions on the home sensing infrastructure without referring either to patient identification data or to the PID. 
Figure~\ref{fig:dataflow} shows how different kinds of data are transferred between entities. This drawing ignores the role of the TelMed entity that, for the time being, can be considered a module of HOS.

%link: https://drive.google.com/file/d/1RISS0KSC2Ixd5tve3gN8NpulcMzMfj9q/view?usp=sharing
%\todo[inline]{I changed the photo to remove the name of OralB and withings}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{img/dataflow-Page-3.drawio.pdf}
    \caption{The dataflow architecture}
    \label{fig:dataflow}
\end{figure}

\textbf{Initialization protocol:} 
\begin{enumerate}
    \item Whenever HOS has a new participating subject with personal data D0, it authenticates itself to the system, generates a PID for that patient, and securely stores the association of PID and D0. An “installation request”  ticket is opened for the IIT with D0 and I\#.
    \item The IIT, when authenticated, will see the ticket and will schedule a first appointment with the subject to visit the apartment and plan the installation. As a result, the IIT will insert some information in the system including the apartment map with the number, type, and planned position of sensors. It will ack the completion through the installation ticket.
    \item The IMT, when authenticated will see the newly enrolled patient with a PID and an installation ticket opened for the corresponding I\#, but it will not have access to any identifying data.  The IMT will prepare the infrastructure equipment, including the HomeGW configured with the subject’s  PID, and, when ready, it will notify the IIT through the ticket.  
    \item The IIT, based on the open ticket, will get the infrastructure devices, schedule an appointment with the subject, and proceed with the installation. When the installation is done, IIT notifies IMT
    \item The  IMT will verify that the whole data acquisition system works as planned and will close the ticket.
    \todo[inline]{I put it as a part of data flow}
    \item Intervention protocol: IMT securely stores I\# with PID. Whenever IMT observes that some data is not being acquired as expected, the connection is interrupted or any other infrastructure is malfunctioning, it sends an intervention request with I\# to IIT  that will send back a notification (with I\#) whenever the problem is solved. Tickets are always closed by the IMT after checking that the issue is solved.
    \item D4 data: \color{Green}Google send the collected D4 data of the subject to the server supporting TDE. The data analysis algorithms will automatically analyze and return the answers to the mentioned questions of clinicians with ID of subject to the HOS. In addition, the results of data analysis of D4 with PID of subject will send to the UniMi for further analyses too. \color{black}
    
\end{enumerate}





\textbf{Pseudonymized DB:} All sensitive data acquired by the Home GW is stored in a database associated with the subject’s PID. The local database is periodically transferred to a central DBMS on the backend in pseudonymized form and the results of data analysis are only associated with the PID.
\textbf{Pseudonymized data re-association:}
The mapping between the PID and the data that HOS uses to identify the subject is stored in a secure storage protected by cryptography (on a DBMS supporting TDE), and will be used by HOS to visualize the data analysis results on a dashboard for the specific subject possibly joined with the subject’s medical records.

%\subsection{Retention policies}

%The retention of sensitive data at the Home GW should be limited not only for storage limitation but more importantly for privacy reasons since it is possibly exposed to IMT. (The current retention is 1 month).
The central DBMS will keep the data for the whole duration of the study. After the study, the data will be anonymized by deleting the association between PID and subject and by performing a further analysis about the risk of reassociating the data with a subject. The anonymized data will be available for further research studies.



%\subsubsection{How outdoor mobility data is collected and structured}
 

%\subsubsection{Obtaining the necessary information without revealing the subject’s identity}

\begin{comment}
    

We explain how we provide the information required by clinicians without revealing the subject’s identity. 
\begin{itemize}
    \item Storing the D4:  Given the sensitivity of these fields, to ensure both privacy and compliance, the collected JSON file should be securely stored in the TDE-enabled table within the database. In addition, before the data is accessible by UniMi for analysis, an automated anonymization algorithm should process the sensitive fields in the dataset.
    \item Strategies for mobility data analysis: The data analysis algorithms are designed to automatically analyze and return the answers to the mentioned questions of clinicians.
\end{itemize}
\end{comment}



\subsection{Compliance with data protection regulations}

\begin{itemize}
    \item Lawfulness, fairness, and transparency: patients provide explicit consent after being clearly informed of the purpose of data collection, the processing methods, and how their information will be utilized. This ensures that the data collection process remains transparent, fair, and lawful~\cite{voigt2017eu}.
    \item Purpose limitation: the collected data is strictly used for the predefined purposes outlined in the consent forms. No data is processed for purposes beyond what is necessary for the execution of the Serenade project.
    \item Data minimization: Only the minimum amount of personal data required to achieve the project’s objectives is collected and processed by each data processor as mentioned in the previous section. 
    \item Storage limitation: personal data is stored only for the duration of the project, after which it is anonymized or deleted, in accordance with retention policies. Sensitive data retained on the home gateway is kept for a limited time to reduce privacy risks. 
    \item Accountability: the system ensures accountability by integrating different techniques (PostgreSQL and Keycloak) which provide essential logging and access control features to log all activities in database and authentication events. 
\end{itemize}






%PostgreSQL logs all database activity, including queries (SELECT) and data modifications (INSERT, UPDATE, DELETE), ensuring that any access to sensitive data (such as patient-id) is tracked. It captures both successful and failed access attempts, allowing administrators to trace user actions and detect any unauthorized activity. This logging mechanism supports full auditing of data access and modification, enhancing the system's security. Keycloak adds an additional layer of accountability through role-based access control (RBAC) and session tracking. It logs authentication events, user roles, and data access permissions, ensuring that only authorized users can access specific data. Each action taken by a user is logged, making it easy to audit access to sensitive information. 









